Engineering Dark Solitary waves in Ring-Trap Bose-Einstein condensates

We demonstrate the feasibility of generation of quasi-stable counter-propagating solitonic structures in an atomic Bose-Einstein condensate confined in a realistic toroidal geometry, and identify optimal parameter regimes for their experimental observation. Using density engineering we numerically identify distinct regimes of motion of the emerging macroscopic excitations, including both solitonic motion along the azimuthal ring direction, such that structures remain visible after multiple collisions even in the presence of thermal fluctuations, and snaking instabilities leading to the decay of the excitations into vortical structures. Our analysis, which considers both mean field effects and fluctuations, is based on the ring trap geometry of Murray et al. Phys. Rev. A 88 053615 2013.

==> Makefile <==
# $Id: Makefile,v 1.9 2009/11/10 19:44:40 youd Exp $
#------------------------------------------------------------------------------
# A Makefile for compiling LaTeX documents.  Written with thesis compilation in
# mind.  Lines to change include:
# * OBJECT: Change this to the name of the main thesis file without extension.
# * BIBTEX: Set this to true if you are using BibTeX for your citations; set it
#           to false otherwise.
# * LATEX: Set this to latex or pdflatex depending on what output format you
#          want and what figure formats are included in your thesis.
# * SOURCES: These are the individual tex files making up the thesis.
#
# Usage:
# make 		- Compile the thesis.  Output depends on the LATEX and BIBTEX
#                 variables.  Default is PS output using BibTeX.
# make twoup 	- Compile as PS but giving output in 2-up format.
# make book 	- Compile as PS but giving output suitable for printing in
# 		  booklet form.  Send to the printer as a duplex job.
# make tidy	- Remove any auxiliary files created during the make process.
# make clean 	- As for make tidy but in addition remove the final output
# 		  files.
#
# Questions/comments to Anthony Youd (a.j.youd@ncl.ac.uk).
#------------------------------------------------------------------------------
OBJECT		= Gallucci_et_al

# Set this variable to true if you are using BibTeX for your citations; set it
# to false otherwise.
BIBTEX		= true

# Set this variable to latex if you are including only PS and EPS figures in
# your thesis; the resulting output will be a PS file.  Set it to pdflatex if
# you are only including PDF, PNG, or JPG images; the resulting output will be
# a PDF file.
LATEX		= latex

# Add list of files here to allow make to only build what is necessary.  Your
# master document should be listed first.
SOURCES		= $(OBJECT).tex \

#---- IMPLICIT RULES ----------------------------------------------------------
.SUFFIXES: .tex .dvi .ps .pdf .ps.gz .bbl

.ps.ps.gz:
	gzip -c $*.ps > $*.ps.gz

.dvi.ps:
	dvips -o $*.ps $*.dvi

.ps.pdf:
	ps2pdf $*.ps

ifeq ($(LATEX), pdflatex)
# Using pdflatex to compile.
.tex.pdf:
	TEXINPUTS=./inputs:$(TEXINPUTS) $(LATEX) --jobname $*_pdf $*
	TEXINPUTS=./inputs:$(TEXINPUTS) $(LATEX) --jobname $*_pdf $*
	TEXINPUTS=./inputs:$(TEXINPUTS) $(LATEX) --jobname $*_pdf $*
	mv $*_pdf.pdf $*.pdf
endif

.tex.dvi:
	TEXINPUTS=./inputs:$(TEXINPUTS) $(LATEX) --jobname $*_dvi $*
	TEXINPUTS=./inputs:$(TEXINPUTS) $(LATEX) --jobname $*_dvi $*
	TEXINPUTS=./inputs:$(TEXINPUTS) $(LATEX) --jobname $*_dvi $*
	mv $*_dvi.dvi $*.dvi

ifeq ($(LATEX), latex)
# Using latex to compile.
.tex.bbl:
	TEXINPUTS=./inputs:$(TEXINPUTS) $(LATEX) --jobname $*_dvi $*
	mv $*_dvi.dvi $*.dvi
	BSTINPUTS=./inputs:$(BSTINPUTS) bibtex $*_dvi
	cp  $*_dvi.bbl  $*.bbl
else
# Using pdflatex to compile.
.tex.bbl:
	TEXINPUTS=./inputs:$(TEXINPUTS) $(LATEX) --jobname $*_pdf $*
	mv $*_pdf.pdf $*.pdf
	BSTINPUTS=./inputs:$(BSTINPUTS) bibtex $*_pdf
	cp  $*_pdf.bbl  $*.bbl
endif

#------------------------------------------------------------------------------
ifeq ($(LATEX), latex)
# Using latex to compile.
default: ps
else
# Using pdflatex to compile.
default: pdf
endif

all: $(OBJECT).dvi ps

#------------------------------------------------------------------------------
ps: $(OBJECT).ps

pdf: $(OBJECT).pdf
	

twoup: $(OBJECT).ps 
	psnup -n2 -Pa4 $(OBJECT).ps $(OBJECT).2up.ps

book: ps
	psbook $(OBJECT).ps book.ps
	psnup -n2 -Pa4 book.ps $(OBJECT).book.ps
	rm -f book.ps

#------------------------------------------------------------------------------
bib:
	rm -f thesis_dvi.bbl
tidy:
	rm -f *.aux *.toc *.log *.out  \
	      *.blg *.idx *.lot *.lof \
	      $(OBJECT)_dvi.* $(OBJECT)_pdf.* */*.aux
clean: tidy
	rm -f $(OBJECT).dvi $(OBJECT).pdf $(OBJECT).ps *.bbl

#---- DEPENDENCIES ------------------------------------------------------------

ifeq ($(BIBTEX), true)
  # With BibTeX
  ifeq ($(LATEX), latex)
    # Using latex to compile.
    $(OBJECT).dvi: $(OBJECT).bbl $(OBJECT).tex $(SOURCES)
  else
    # Using pdflatex to compile.
    $(OBJECT).pdf: $(OBJECT).bbl $(OBJECT).tex $(SOURCES)
  endif
else
  # Without BibTeX
  ifeq ($(LATEX), latex)
    # Using latex to compile.
    $(OBJECT).dvi: $(OBJECT).tex
  else
    # Using pdflatex to compile.
    $(OBJECT).pdf: $(OBJECT).tex
  endif
endif

$(OBJECT).bbl: $(OBJECT).tex Gallucci_et_al.bib $(SOURCES)
$(OBJECT).ps: $(OBJECT).dvi
$(OBJECT).ps.gz: $(OBJECT).ps

